A tractable formulation for multi-period linearized optimal power flow in presence of thermostatically controlled loads

This paper presents a convex reformulation of a nonlinear constrained optimization problem for Markov decision processes, and applies the technical findings to optimal control problems for an ensemble of thermostatically controlled loads (TCLs). The paper further explores the formulation and solution of a (linearized) AC optimal power flow problem when one or more ensembles of TCLs are connected to a power network. In particular, a receding horizon controller is proposed, to simultaneously compute the optimal set-points of distributed energy resources (DERs) in the grid and the optimal switching signal for the TCLs. This formulation takes into account hardware constraints of the DERs, operational constraints of the grid (e.g., voltage limits), comfort of the TCL users, and ancillary services provision at the substation. Numerical results are provided to verify the effectiveness of the proposed methodology.

==> Tikz_common_styles.tex <==
%_______________________________________________________________
%
%     Tikz_common_styles
%
%     TikZ styles for drawing block diagrams.
%
%      Roy Smith,  15 July 2014
%
%_______________________________________________________________
\typeout{Reading Tikz styles:  Tikz_common_styles}
%
%   Block diagram styles
\tikzstyle{block} = [draw,rectangle,thick,minimum height=2em,minimum width=1.0cm,
                                top color=blue!10, bottom color=blue!10]%
\tikzstyle{sum} = [draw,circle,inner sep=0mm,minimum size=2mm]%
\tikzstyle{connector} = [->,thick]%
\tikzstyle{line} = [thick]%
\tikzstyle{branch} = [circle,inner sep=0pt,minimum size=1mm,fill=black,draw=black]%
\tikzstyle{guide} = []%
%
%   colours for various blocks
\tikzstyle{deltablock} = [block, top color=red!10, bottom color=red!10]%
\tikzstyle{controlblock} = [block, top color=green!10, bottom color=green!10]%
\tikzstyle{weightblock} = [block, top color=orange!10, bottom color=orange!10]%
\tikzstyle{clpblock} = [block, top color=cyan!10, bottom color=cyan!10]%
%
%  styles for dimming block components.
\tikzstyle{block_dim} = [draw,rectangle,thick,minimum height=2em,minimum width=2em,
                                color=black!15]%
\tikzstyle{sum_dim} = [draw,circle,inner sep=0mm,minimum size=2mm,color=black!15]%
\tikzstyle{connector_dim} = [->,thick,color=black!15]%
%
%    Graph styles
\tikzstyle{smalllabel} = [font=\footnotesize]%
\tikzstyle{axiswidth}=[semithick]%
\tikzstyle{axiscolor}=[color=black!50]%
\tikzstyle{help lines} =[color=blue!40,very thin]%
\tikzstyle{axes} = [axiswidth,axiscolor,<->,smalllabel]%
\tikzstyle{axis} = [axiswidth,axiscolor,->,smalllabel]%
\tikzstyle{tickmark} = [thin,smalllabel]%
\tikzstyle{plain_axes} = [axiswidth,smalllabel]%
\tikzstyle{w_axes} = [axiswidth,->,smalllabel]%
\tikzstyle{m_axes} = [axiswidth,smalllabel]%
\tikzstyle{dataplot} = [thick]%
%
%_______________________________________________________________


==> commands.tex <==
%%%%%% Fernando's commands %%%%%%%%%%%%

%%\input{psfig}
%\setlength{\textwidth}{6.5 in}
%\setlength{\oddsidemargin}{0 in}
%\setlength{\evensidemargin}{0 in}

% xfig shit
%\newcommand{\tenrm}{\relax}
%\newcommand{\ninrm}{\relax}
%\newcommand{\sevrm}{\relax}
%\newcommand{\svtnrm}{\relax}
%\newcommand{\twlrm}{\relax}
%\newcommand{\twfvrm}{\relax}
%\newcommand{\frtnrm}{\relax}
%\newcommand{\ninbf}{\relax}

% Theorems, etc; this version uses different numbering for each case.
%\newtheorem{theorem}{Theorem}
%\newtheorem{corollary}{Corollary}
%\newtheorem{lemma}{Lemma}
%\newtheorem{proposition}{Proposition}
%\newtheorem{definition}{Definition}
%\newtheorem{remark}{Remark}
%\newtheorem{example}{Example}

% Theorems, unified numbering
%\newtheorem{theorem}{Theorem}
%\newtheorem{corollary}[theorem]{Corollary}
%\newtheorem{lemma}[theorem]{Lemma}
%\newtheorem{proposition}[theorem]{Proposition}
%\newtheorem{definition}{Definition}
%\newtheorem{remark}{Remark}
%\newtheorem{problem}{Problem}
%\newtheorem{example}{Example}
%\newtheorem{condition}{Condition}


%Space

\newcommand{\vmo}{\vspace{-1ex}}
\newcommand{\vmt}{\vspace{-2ex}}
\newcommand{\vmth}{\vspace{-3ex}}
\newcommand{\vpo}{\vspace{1ex}}
%\newcommand{\vpt}{\vspace{2ex}}
\newcommand{\vpth}{\vspace{3ex}}

% Command abbreviations

\newcommand{\enma}[1]   {\ensuremath{#1}}
\newcommand{\noi}{\noindent}
\newcommand{\non}{\nonumber}

\newcommand{\reo}[1]{(\ref{#1})}
\newcommand{\reeq}[1]{(\ref{eq.#1})}
\newcommand{\reex}[1]{(\ref{ex.#1})}
\newcommand{\reeqs}[2]{(\ref{eq.#1}-\ref{eq.#2})}
\newcommand{\refi}[1]{Figure \ref{fig.#1}}
\newcommand{\reth}[1]{Theorem \ref{teo.#1}}
\newcommand{\relem}[1]{Lemma \ref{lemma.#1}}
\newcommand{\repro}[1]{Proposition \ref{prop.#1}}
\newcommand{\resec}[1]{Section \ref{sec.#1}}
\newcommand{\ressec}[1]{Section \ref{ssec.#1}}
\newcommand{\recha}[1]{Chapter \ref{cha.#1}}
\newcommand{\recond}[1]{Condition \ref{cond.#1}}
\newcommand{\recoro}[1]{Corollary \ref{corol.#1}}
\newcommand{\reapp}[1]{Appendix \ref{append.#1}}
\newcommand{\refdef}[1]{Definition \ref{def.#1}}
\newcommand{\redef}[1]{Definition \ref{def.#1}}

\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\bseq}{\begin{subequations}}
\newcommand{\eseq}{\end{subequations}}
\newcommand{\beqn}{\begin{eqnarray}}
\newcommand{\eeqn}{\end{eqnarray}}
\newcommand{\ba}{\begin{array}}
\newcommand{\ea}{\end{array}}
\newcommand{\bct}{\begin{center}}
\newcommand{\ect}{\end{center}}
\newcommand{\btab}{\begin{tabular}}
\newcommand{\etab}{\end{tabular}}
\newcommand{\btmz}{\begin{itemize}}
\newcommand{\etmz}{\end{itemize}}
\newcommand{\benum}{\begin{enumerate}}
\newcommand{\eenum}{\end{enumerate}}

%\newcommand{\bal}{\begin{align}}
%\newcommand{\eal}{\end{align}}

\newcommand{\flecha}{{\rightarrow}}
\newcommand{\flechah}[1]{\stackrel{#1\rightarrow 0}{\longrightarrow}}
\newcommand{\flechahp}[1]{\stackrel{#1\rightarrow 0+}{\longrightarrow}}
\newcommand{\flechas}[2]{\stackrel{\stackrel{#1\rightarrow 0}{#2\rightarrow 0}}{\longrightarrow}}
\newcommand{\flechaN}[1]{\stackrel{#1\rightarrow\infty}{\longrightarrow}}
%\newcommand{\flechaN}{\stackrel{N\rightarrow\infty}{\longrightarrow}}
\newcommand{\implica}{{\Rightarrow}}
\newcommand{\Implica}{{\Longrightarrow}}
\newcommand{\sii}{{\Leftrightarrow}}
\newcommand{\Sii}{{\Longleftrightarrow}}


% For proofs

%\newcommand{\proof}{{\sc Proof.\ }}
%\Newcommand{\pfbox}{\hfill\mbox{$\Box$}}
\newcommand{\defequal}{:=}
\newcommand{\ha}{\frac{1}{2}}
%\newcommand{\eopr}{\begin{flushright} $\Box$ \end{flushright}}
\newcommand{\eopr}{\hfill \rule{1.2ex}{1.2ex}}
\newcommand{\chico}{\scriptscriptstyle}
%\newenvironment{pf}{\paragraph*{Proof{\rm.}}}{\pfbox\bigskip}


%Gral. notation, function spaces

\newcommand{\R}{{\mathbb R}}
\newcommand{\C}{{\mathbb C}}
\newcommand{\Z}{{\mathbb Z}}
\newcommand{\T}{{\mathbb T}}
\newcommand{\V}{{\mathbb V}}
\newcommand{\G}{{\mathbb G}}
\newcommand{\hG}{\hat{\G}}
\newcommand{\W}{{\mathbb W}}
\newcommand{\D}{{\mathbb D}}
\newcommand{\beh}{{\mathcal B}}
\newcommand{\beheps}{{\mathcal B}_{\epsilon}}
\newcommand{\sT}{{ {\bf T}}}
\newcommand{\F}{{\mathbb F}}
\newcommand{\Fou}{{\mathcal F}}
\newcommand{\X}{{\mathbb X}}
\newcommand{\Xb}{\mbox{\boldmath $\mathit{X}$}}
%\newcommand{\X}{{\bf X}}
\newcommand{\ques}{\cal {\bf Q}}



\newcommand{\lam}{\enma{\lambda}}
\newcommand{\cH}{\enma{\mathcal H}}
\newcommand{\cL}{\enma{\mathcal L}}
\newcommand{\cF}{\enma{\mathcal F}}
\newcommand{\Flti}{\enma{\mathcal F^{\chico LTI}}}
\newcommand{\clc}{\enma{\mathcal L}_c}
\newcommand{\smax}[1] { \bar \sigma \left( #1 \right) }
%\newcommand{\smax} { \bar{\sigma}}
\newcommand{\smin}[1] { \underline{\sigma} \left( #1 \right) }
\newcommand{\norm}[1]{\| #1 \|}                 %does not make large \|
\newcommand{\Norm}[1]{\left\| #1 \right\|}
\newcommand{\Hinf}{\mathcal{H}_{\infty} }
\newcommand{\Ht}{ \mathcal{H}_{2}}
\newcommand{\Htprp}{  \mathcal{H}_{2}^{\perp} }
\newcommand{\RHt}{  \mathcal{RH}_{2} }
\newcommand{\RHtprp}{  \mathcal{RH}_{2}^{\perp} }
\newcommand{\RHinf}{  \mathcal{RH}_{\infty} }
\newcommand{\Lt}{  \mathcal{L}_2 }
\newcommand{\RLt}{  \mathcal{RL}_{2} }
\newcommand{\Lone}{  \mathcal{L}_1 }
\newcommand{\lone}{l_1 }
%\newcommand{\lt}{  l_2 }
\newcommand{\lte}{  l_{2e} }
\newcommand{\Lte}{  \mathcal{L}_{2e} }
\newcommand{\Linf}{  \mathcal{L}_{\infty} }
\newcommand{\RLinf}{  \mathcal{RL}_{\infty} }
\newcommand{\Ltplusd}{ \mathcal{L}_2  [0, \infty ) }
\newcommand{\Ltplus}{ \mathcal{L}_{2+} }
\newcommand{\Pplus}{ P_{+} }
\newcommand{\Ltminusd}{ \mathcal{L}_2 (-\infty ,0] }
\newcommand{\Ltminus}{ \mathcal{L}_{2-}}
\newcommand{\Pminus}{ P_{-} }
\newcommand{\nab}{{\bf \nabla}}
\newcommand{\nabo}{{\bf \nabla}^0}
\newcommand{\w}{\omega}
\newcommand{\dospi}{\frac{1}{2\pi}}
\newcommand{\unopi}{\frac{1}{\pi}}
\newcommand{\betapi}{\frac{\beta}{\pi}}
\newcommand{\Bpi}{\frac{B}{\pi}}
\newcommand{\wpi}{\frac{\w}{\pi}}
\newcommand{\dw}{\frac{d\omega}{2\pi}}
\newcommand{\ejw}{ e^{j\omega} }
\newcommand{\ejs}{ e^{js} }
\newcommand{\fnu}{\mbox{\boldmath $B^{\nu}$}}
\newcommand{\fnubar}{\mbox{\boldmath $B^{\bar{\nu}}$}}
%\newcommand{\fnu}{\enma{\mbox{\boldmath $\mathcal{F}$}(\nu)}\xspace}
%\newcommand{\fnubar}{\enma{\mbox{\boldmath $\mathcal{F}$}(\bar{\nu})}\xspace}
%\newcommand{\fnu}{{\cal F}(\nu)}
\newcommand{\intinf}{\int_{-\infty}^{\infty}}


\newcommand{\ws}{\w_1,\ldots,\w_d}
\newcommand{\Llt}[1]{{\cal L}(l_2^{#1})}
\newcommand{\thetas}{\theta^1,\ldots,\theta^d}
\newcommand{\vs}{v^1,\ldots,v^d}
\newcommand{\xfi}{X^\Phi}
\newcommand{\xth}{X^\theta}
\newcommand{\Xfi}{\X^\Phi}
\newcommand{\Xth}{\X^\theta}





%\newcommand{\diag}      {\enma{\mathrm{diag}}}
\newcommand{\Ker}       {\enma{\mathrm{Ker}}}
\newcommand{\trace}     {\enma{\mathrm{trace}}}
\newcommand{\co}        {\enma{\mathrm{co}}}
\newcommand{\col}       {\enma{\mathrm{col}}}
\newcommand{\rad}       {\enma{\mathrm{rad}}}
\newcommand{\blockdiag} {\enma{\mathrm{blockdiag}}}
\newcommand{\eig}       {\enma{\mathrm{eig}}}
\newcommand{\sgn}       {\enma{\mathrm{sgn}}}
\newcommand{\re}        {\enma{\mathrm{Re}}}
\newcommand{\im}        {\enma{\mathrm{Im}}}
\newcommand{\defeq}     {\enma{\;\triangleq\;}}
\newcommand{\then}      {\enma{\;\Longrightarrow\;}}
\newcommand{\neth}      {\enma{\;\Longleftarrow\;}}
\newcommand{\inner}[2]{\left\langle #1,#2 \right\rangle}










% Operators, transfer functions

%\newcommand{\op}[1]{ \mbox{\boldmath $ #1$}}
%\newcommand{\tf}[1]{ \enma{\hat{#1}}}
%\newcommand{\opdel}{\mbox{\boldmath $\mathit{\Delta}$}}





\newcommand{\ahat}{\hat{A}}
\newcommand{\bhat}{\hat{B}}
\newcommand{\chat}{\hat{C}}
\newcommand{\dhat}{\hat{D}}
\newcommand{\rhat}{\hat{R}}
\newcommand{\qhat}{\hat{Q}}
\newcommand{\phat}{\hat{P}}
\newcommand{\psih}{\hat{\psi}}
\newcommand{\hv}{\hat{v}}
\newcommand{\homega}{\hat{\omega}}
\newcommand{\hu}{\hat{u}}
\newcommand{\hw}{\hat{w}}
\newcommand{\hp}{\hat{p}}
\newcommand{\hd}{\hat{d}}
\newcommand{\bv}{\bar{v}}
\newcommand{\bomega}{\bar{\omega}}




\newcommand{\ahatlam}{\hat{A}(\lam)}
\newcommand{\bhatlam}{\hat{B}(\lam)}
\newcommand{\chatlam}{\hat{C}(\lam)}
\newcommand{\dhatlam}{\hat{D}(\lam)}
\newcommand{\rhatlam}{\hat{R}(\lam)}
\newcommand{\qhatlam}{\hat{Q}(\lam)}






\newcommand{\tf}[1]{\enma{#1}}
\newcommand{\op}[1]{\enma{\mathbf{#1}}}
\newcommand{\opm}{\op{M}\xspace}
\newcommand{\opl}{\op{L}\xspace}
\newcommand{\opi}{\op{I}\xspace}
\newcommand{\opzero}{\op{0}\xspace}
\newcommand{\opk}{\op{K}\xspace}
\newcommand{\opd}{\op{D}\xspace}
\newcommand{\oph}{\op{H}\xspace}
\newcommand{\opat}{\op{A}^T\xspace}
\newcommand{\opg}{\op{G}\xspace}
\newcommand{\opf}{\op{F}\xspace}
\newcommand{\opp}{\op{P}\xspace}
\newcommand{\opn}{\op{N}\xspace}
\newcommand{\opq}{\op{Q}\xspace}
\newcommand{\opr}{\op{R}\xspace}
\newcommand{\ops}{\op{S}\xspace}
\newcommand{\opt}{\op{T}\xspace}
\newcommand{\opu}{\op{U}\xspace}
\newcommand{\opv}{\op{V}\xspace}

\newcommand{\opdel}{\op{\del}\xspace}
\newcommand{\opups}{\op{\Upsilon}\xspace}
\newcommand{\opdelbar}{\op{\bar{\del}}\xspace}
\newcommand{\opdelhat}{\op{\hat{\del}}\xspace}
\newcommand{\opdelhatk}{\op{\hat{\del}}^k\xspace}
\newcommand{\opdelbart}{\op{\bar{\del}}^T\xspace}
\newcommand{\opdelta}{\mbox{\boldmath $\delta$}\xspace}
\newcommand{\oplam}{\mbox{\boldmath $\lam$}\xspace}
\newcommand{\opphi}{\op{\Phi}\xspace}
\newcommand{\oppsi}{\op{\Psi}\xspace}
\newcommand{\optheta}{\mbox{\boldmath $\theta$}\xspace}
\newcommand{\opthetachico}{\mbox{\small\boldmath $\theta$}\xspace}
\newcommand{\opvarrho}{\mbox{\boldmath $\varrho$}\xspace}








%deltas
\newcommand{\del}{\Delta}
\newcommand{\ddel}{{\bf \Delta}}
\newcommand{\ddelti}{{\bf \Delta^{\scriptscriptstyle LTI}}}
\newcommand{\ddeltv}{{{\bf \Delta^{\scriptscriptstyle LTV}}}}
\newcommand{\ddelslow}{{\bf \Delta^{\nu}}}
\newcommand{\bdelti}{{\bf B_{\Delta^{\scriptscriptstyle LTI}}}}
\newcommand{\bdeltv}{{\bf B_{\Delta^{\scriptscriptstyle LTV}}}}
\newcommand{\bdelnl}{{\bf B_{\Delta^{\scriptscriptstyle NL}}}}
\newcommand{\bdelslow}{{\bf B_{\Delta^\nu}}}
\newcommand{\bdeluno}{{\bf B_{\Delta_1}}}
\newcommand{\bdeldos}{{\bf B_{\Delta_2}}}
\newcommand{\delo}{\Delta_0}
\newcommand{\ddelo}{{\bf \Delta_0}}
\newcommand{\Bdel}{{\bf B_{\Delta}}}
\newcommand{\Bdelo}{{\bf B_{\Delta_0}}}
\newcommand{\delu}{\Delta_{u}}
\newcommand{\ddelu}{{\bf \Delta_{u}}}
\newcommand{\Bdelu}{{\bf B_{\Delta_{u}}}}
\newcommand{\dels}{\Delta_{S}}
\newcommand{\ddels}{{\bf \Delta_{S}}}
\newcommand{\Bdels}{{\bf B_{\Delta_{S}}}}
\newcommand{\delso}{\Delta_{S_0}}
\newcommand{\ddelso}{{\bf \Delta_{S_0}}}
\newcommand{\Bdelso}{{\bf B_{\Delta_{S_0}}}}
\newcommand{\bvarrho}{\mathbf{B_\varrho}}



%White noise stuff

\newcommand{\Wngt}{W_{N,\gamma,T}}
\newcommand{\Wnt}{W_{N,T}}
\newcommand{\Wng}{W_{N,\gamma}}
\newcommand{\Wgt}{W_{\gamma,T}}
\newcommand{\Wt}{W_{T}}
\newcommand{\BP}{\cal BP}
\newcommand{\subN}{_{\scriptscriptstyle N}}
\newcommand{\subF}{_{\scriptscriptstyle F}}
\newcommand{\Fch}{{\scriptscriptstyle F}}


\newcommand{\WFnav}{\hat{W}_{N,\alpha,V}} %freq domain set
\newcommand{\Wneta}{\hat{W}_{N,\eta}} %freq domain set
\newcommand{\Weta}{\hat{W}_{\eta}} %freq domain set
\newcommand{\Setab}{S_{\eta,B}} %freq domain set
\newcommand{\Wetab}{W_{\eta,B}} %freq domain set
\newcommand{\WFav}{\hat{W}_{\alpha,V}} %freq domain set
\newcommand{\prob}[1]{{\cal P}\left( #1 \right)}


% Analysis stuff

\newcommand{\Cprp}{C_{\perp}}
\newcommand{\Csprp}{C_{S\perp}}
\newcommand{\Cuprp}{C_{u\perp}}


% Mixed LTI/LTV stuff

\newcommand{\pphi}{{\bf \Phi}}
\newcommand{\ppsi}{{\bf \Psi}}
\newcommand{\ttheta}{{\Theta}}
\newcommand{\ddelta}{{\mathbb \delta}}
\newcommand{\bpphi}{{\bf B}_{\pphi}}
\newcommand{\bppsi}{{\bf B}_{\ppsi}}
\newcommand{\bttheta}{{\bf B}_{\ttheta}}
\newcommand{\bddelta}{{\bf B_\delta}}
\newcommand{\phit}{\tilde{\Phi}}
\newcommand{\psit}{\tilde{\Psi}}
\newcommand{\pphit}{{\bf \tilde{\Phi}}}
\newcommand{\delt}{\tilde{\del}}
\newcommand{\ddelt}{{\bf \tilde{\del}}}
\newcommand{\bdelt}{{\bf B}_\ddelt}
\newcommand{\atil}{\tilde{A}}
\newcommand{\mtil}{\tilde{M}}
\newcommand{\htil}{\tilde{H}}
\newcommand{\ctil}{\tilde{C}}
\newcommand{\gtil}{\tilde{G}}
\newcommand{\ftil}{\tilde{F}}
\newcommand{\vtil}{\tilde{v}}



%Array stuff

% Sets uniform spacing for all matrices. To avoid it just comment out
% the renewcommand stuff

\newcommand{\matbegin}{
%       \renewcommand{\baselinestretch}{1.5}
%       \renewcommand{\arraystretch}{0.7}
        \left[
}
\newcommand{\matend}{
        \right]
}



\newcommand{\tbo}[2]{
  \matbegin \begin{array}{c}
       #1 \\ #2
       \end{array} \matend }
\newcommand{\thbo}[3]{
  \matbegin \begin{array}{c}
       #1 \\ #2 \\ #3
       \end{array} \matend }
\newcommand{\obt}[2]{
  \matbegin \begin{array}{cc}
       #1 & #2
       \end{array} \matend }
\newcommand{\obth}[3]{
  \matbegin \begin{array}{ccc}
       #1 & #2 & #3
       \end{array} \matend }
\newcommand{\tbt}[4]{
  \matbegin \begin{array}{cc}
       #1 & #2 \\ #3 & #4
       \end{array} \matend }
\newcommand{\thbt}[6]{
  \matbegin \begin{array}{cc}
       #1 & #2 \\ #3 & #4 \\ #5 & #6
       \end{array} \matend }
\newcommand{\tbth}[6]{
  \matbegin \begin{array}{ccc}
       #1 & #2 & #3\\ #4 & #5 & #6
       \end{array} \matend }
\newcommand{\thbth}[9]{
 \matbegin \begin{array}{ccc}
                #1 & #2 & #3 \\
                #4 & #5 & #6 \\
                #7 & #8 & #9
                \end{array}\matend}
\newcommand{\fbo}[4]{
 \matbegin \begin{array}{c}
                #1 \\ #2 \\ #3 \\ #4
                \end{array}\matend}
\newcommand{\obf}[4]{
 \matbegin \begin{array}{cccc}
                #1 & #2 & #3 & #4
                \end{array}\matend}
\newcommand{\fvbo}[5]{
 \matbegin \begin{array}{c}
                #1 \\ #2 \\ #3 \\ #4 \\ #5
                \end{array}\matend}
\newcommand{\obfv}[5]{
 \matbegin \begin{array}{ccccc}
                #1 & #2 & #3 & #4 & #5
                \end{array}\matend}

\newcommand{\tbtb}[4]{
  \matbegin \begin{array}{cc}  \displaystyle
       #1 &  \displaystyle #2 \\  \displaystyle #3 &  \displaystyle #4
       \end{array} \matend }

%\newcommand{\fbf}[16]{
%  \matbegin \begin{array}{cccc}
%        #1 &  #2 &  #3 &  #4 \\
%        #5 &    #6 &   #7 &    #8 \\
%        #9 &    #10 &   #11 &    #12 \\
%        #13 &    #14 &   #15 &    #16
%       \end{array}
%       \matend }


\newcommand{\stsp}[4]{  \matbegin \begin{array}{c|c}
       #1 & #2 \\ \hline
       #3 & #4
       \end{array} \matend }

\newcommand{\stsptbth}[6]{  \matbegin \begin{array}{c|cc}
       #1 & #2 & #3\\ \hline
       #4 & #5 & #6
       \end{array} \matend }

\newcommand{\stspthbt}[6]{  \matbegin \begin{array}{c|c}
       #1 & #2 \\ \hline
       #3 & #4 \\
       #5 & #6
       \end{array} \matend }

\newcommand{\stspthbth}[9]{  \matbegin \begin{array}{c|cc}
        #1 & #2 & #3 \\ \hline
        #4 & #5 & #6 \\
        #7 & #8 & #9
       \end{array} \matend }


% Sets smaller spacing for matrices inside text; to avoid it just comment out
% the renewcommand stuff

\newcommand{\matparbegin}{
        \renewcommand{\baselinestretch}{1}
        \renewcommand{\arraystretch}{.5}
        \setlength{\arraycolsep}{.25em}
        \left[
}
\newcommand{\matparend}{
        \right]
}

%Two by one, two by two, two by three inside paragraph.

\newcommand{\tbopar}[2]{
  \matparbegin \begin{array}{c}
       #1 \\ #2
       \end{array} \matparend }


\newcommand{\obtpar}[2]{
  \matparbegin \begin{array}{cc}
       #1 & #2
       \end{array} \matparend }


\newcommand{\tbtpar}[4]{
  \matparbegin \begin{array}{cc}
       #1 & #2 \\ #3 & #4
       \end{array} \matparend }

\newcommand{\tbthpar}[6]{
  \matparbegin \begin{array}{ccc}
       #1 & #2 & #3\\ #4 & #5 & #6
       \end{array} \matparend }

% Sets intermediate  spacing for matrices; to avoid it just comment out
% the renewcommand stuff

\newcommand{\matintbegin}{
        \renewcommand{\baselinestretch}{1}
        \renewcommand{\arraystretch}{.7}
        \setlength{\arraycolsep}{.3em}
        \left[
}
\newcommand{\matintend}{
        \right]
}

%Intermediate two by one, two by two, two by three

\newcommand{\tboint}[2]{
  \matintbegin \begin{array}{c}
       #1 \\ #2
       \end{array} \matintend }

\newcommand{\obtint}[2]{
  \matintbegin \begin{array}{cc}
       #1 & #2
       \end{array} \matintend }


\newcommand{\tbtint}[4]{
  \matintbegin \begin{array}{cc}
       #1 & #2 \\ #3 & #4
       \end{array} \matintend }

\newcommand{\tbthint}[6]{
  \matintbegin \begin{array}{ccc}
       #1 & #2 & #3\\ #4 & #5 & #6
       \end{array} \matintend }






%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Bassam's defs ( afew are commented out)










\newcommand{\dhoo}{\hat{D}_{11}}
\newcommand{\ca}{{\cal A}}
\newcommand{\hca}{\hat{\cal A}}
\newcommand{\cq}{{\cal Q}}
\newcommand{\calo}{{\cal O}}
\newcommand{\ce}{{\cal E}}
\newcommand{\inv}[1]{#1^{\scriptscriptstyle -1}}
\newcommand{\wctau}{W_\tau}
\newcommand{\bbee}{{\rm \bf b}}
\newcommand{\cabe}{{\cal B}}
\newcommand{\cace}{{\cal C}}
\newcommand{\lonen}{\ell^1(n)}
\newcommand{\linfn}{\ell^\infty (n)}
\newcommand{\bhst}{ ^*\hat{B}_1}
\newcommand{\hsli}{({\cal H}_n{\cal S}_n)^{\scriptscriptstyle -L}}
\newcommand{\hjli}{({\cal H}_n{\cal J}_n)^{\scriptscriptstyle -L}}
\newcommand{\hs}{({\cal H}_n{\cal S}_n)}
\newcommand{\hj}{({\cal H}_n{\cal J}_n)}
\newcommand{\cln}{{\cal L}_n}
\newcommand{\oh}{\hat{\cal O}}
\newcommand{\oho}{\hat{\cal O}_o}
\newcommand{\fdbk}[2]{{\cal F}(#1,#2)}
\newcommand{\elft}{\ell^\infty_{L^\infty {\scriptscriptstyle [0,\tau]}}}
\newcommand{\elinf}{\ell_{L^\infty {\scriptscriptstyle [0,\tau]}}}
\newcommand{\Lft}{L^\infty {\scriptstyle [0,\infty]}}
\newcommand{\Lfte}{L^\infty_e {\scriptstyle [0,\infty]}}
\newcommand{\Lftt}{L^\infty {\scriptstyle [0,\tau]}}
\newcommand{\Lonet}{L^1 {\scriptstyle [0,\tau]}}
\newcommand{\elone}{\ell^1}
\newcommand{\elfn}{\ell^\infty {\scriptstyle (n)}}
\newcommand{\inn}{{\cal J}_n}
\newcommand{\inntl}{\tilde{\cal J}_n}
\newcommand{\hon}{{\cal H}_n}
\newcommand{\san}{{\cal S}_n}
\newcommand{\hot}{{\cal H}_\tau}
\newcommand{\sat}{{\cal S}_\tau}
\newcommand{\hoth}{\hat{\cal H}_\tau}
\newcommand{\sath}{\hat{\cal S}_\tau}
\newcommand{\dis}{I \hspace*{-.42em}{\cal D}_\tau}
\newcommand{\imb}{I \hspace*{-.41em}I}
\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\cell}{{\cal L}}
\newcommand{\ttl}{\tilde{T}}
\newcommand{\rtl}{\tilde{R}}
\newcommand{\ftl}{\tilde{f}}
\newcommand{\calc}{{\cal C}}
\newcommand{\cali}{{\cal I}}
\newcommand{\calg}{\G}
\newcommand{\fbr}{\bar{f}}
\newcommand{\coh}{\hat{{\cal O}}}
\newcommand{\xdot}{\dot{x}}
\newcommand{\enex}{{n_x}}
\newcommand{\enu}{{n_u}}
\newcommand{\eny}{{n_y}}

\newcommand{\cd}{\hat{{\cal D}}}
\newcommand{\cs}{{\cal S}}



\newcommand{\ra}{\rightarrow}
\newcommand{\peee}{(I-\hat{D}_{11}\hat{D}_{11}^*)}
\newcommand{\ess}{(I-\hat{D}_{11}^* \hat{D}_{11})}
\newcommand{\tpee}{(I-TT^*)^{1/2}}
\newcommand{\tess}{(I-T^*T)^{1/2}}
\newcommand{\Ltwo}{L^2[0,\tau]}
\newcommand{\nb}{{\cal N}(\bar{B}_1)}
\newcommand{\rng}[1]{{\cal R}{\scriptstyle ( #1 )}}
\newcommand{\rcd}{{\cal R}(\bar{C}_1,\bar{D}_{12})}
\newcommand{\ustp}[1]{{\bf 1} \hspace*{-.12em}{\scriptstyle( #1 )}\hspace*{.08em}}
\newcommand{\hif}{H^\infty}
%\newcommand{\del}{\mbox{${\bf \Delta} \hspace*{-.83em}\Delta$}}
\newcommand{\ifnm}[1]{\mbox{$ \|#1\|_{H^\infty}$}}
\newcommand{\anm}[1]{\mbox{$ \|#1\|_{\cal A} $}}
\newcommand{\real}{\R}
\newcommand{\arr}{{I \hspace*{-.3em}R}}
\newcommand{\cplx}{\mbox{$ | \hspace*{-.4em}C$}}
\newcommand{\cplxs}{ C\kern -.35em \rule{0.03 em}{.7 ex}~   }
\newcommand{\integ}{\Z}
\def\complex{\hbox{C\kern -.45em \rule{0.03 em}{1.5 ex}}~}
\newcommand{\numb}{\mbox{$ I \hspace*{-.4em}N$}}
\newcommand{\lra}{\longrightarrow}
\newcommand{\lla}{\mbox{$\longleftarrow$}}
%\newcommand{\Lt}{L^p[0,\tau]}
\newcommand{\elt}{\mbox{$\ell^p_{L^p[0,\tau]}$}}
\newcommand{\eltwo}{\mbox{$\ell^2_{L^2[0,\tau]}$}}
\newcommand{\wt}{W_\tau}
\newcommand{\wit}{W_\tau^{-1}}
\newcommand{\gh}{\mbox{$\hat{G}$}}
\newcommand{\gtl}{\mbox{$\tilde{G}$}}
\newcommand{\gbr}{\bar{G}}
\newcommand{\gbrev}{\breve{G}}
\newcommand{\gcute}{\acute{G}}
\newcommand{\tcute}{\acute{T}}
%\newcommand{\th}{\hat{t}}
%\newcommand{\Th}{\hat{T}}
\newcommand{\sh}{\hat{s}}
%%\newcommand{\fh}{\hat{f}}
\newcommand{\rh}{\hat{r}}
\newcommand{\uh}{\hat{u}}
\newcommand{\xh}{\hat{x}}
\newcommand{\yh}{\hat{y}}
\newcommand{\ah}{\hat{A}}
\newcommand{\bh}{\hat{B}}
\newcommand{\ch}{\hat{C}}
%\newcommand{\dh}{\hat{D}}
\newcommand{\atl}{\tilde{A}}
\newcommand{\btl}{\tilde{B}}
\newcommand{\ctl}{\tilde{C}}
\newcommand{\dtl}{\tilde{D}}
\newcommand{\abr}{\bar{A}}
\newcommand{\bbr}{\bar{B}}
\newcommand{\cbr}{\bar{C}}
\newcommand{\dbr}{\bar{D}}
\newcommand{\bbrev}{\breve{B}}
\newcommand{\cbrev}{\breve{C}}
\newcommand{\dbrev}{\breve{D}}
\newcommand{\aacute}{\acute{A}}
\newcommand{\bcute}{\acute{B}}
\newcommand{\ccute}{\acute{C}}
\newcommand{\dcute}{\acute{D}}
\newcommand{\bbrh}{\hat{\bar{B}}}
\newcommand{\wtl}{\tilde{w}}
\newcommand{\ztl}{\tilde{z}}
\newcommand{\wh}{\hat{w}}
\newcommand{\zh}{\hat{z}}
\newcommand{\ytl}{\tilde{y}}
\newcommand{\utl}{\tilde{u}}
\newcommand{\chtwo}{\mbox{${\cal H}^2_{L^2[0,\tau]}$}}
\newcommand{\hinf}{{\cal H}^\infty}
\newcommand{\echt}{{\cal H}^2}
\newcommand{\hths}{{\cal H}^2_{{\rm HS}}}

\newcommand{\bi}{\begin{itemize}}
\newcommand{\ei}{\end{itemize}}

\def\calF{{\cal{F}}}
\def\hatz{\hat{z}}
\def\hatdelta{\hat{\delta}}
\def\hattheta{\hat{\theta}}
\def\barsigma{\bar{\sigma}}
\def\barz{\bar{z}}
%\newcommand{\diag}[3]{\mbox{diag}\left[ #1, #2, #3 \right]}
\newcommand{\diagfour}[4]{\mbox{diag}\left[ #1, #2, #3, #4 \right]}
\newcommand{\pbp}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\pbpt}[2]{\frac{\partial^2 #1}{\partial #2^2}}
\newcommand{\der}[2]{ \frac{ \partial #1}{ \partial #2} }
\newcommand{\dder}[2]{ \dfrac{ \partial #1}{ \partial #2} }
\newcommand{\dert}[2]{ \frac{\partial^2 #1}{ \partial #2^2} }



\newcommand{\system}[4]{
 \left[
  \begin{array}{c|c}
   #1 & #2 \\
   \hline
   #3 & #4
  \end{array}
 \right]
  }
\newcommand{\systemb}[9]{
 \left[
  \begin{array}{cc|c}
   #1 & #2 & #3   \\
   #4 & #5 & #6   \\
   \hline
   #7 & #8 & #9
  \end{array}
 \right]
  }
\newcommand{\systembd}[9]{
 \left[
  \begin{array}{c|cc}
   #1 & #2 & #3   \\
   \hline
   #4 & #5 & #6   \\
   #7 & #8 & #9
  \end{array}
 \right]
  }

\newcommand{\tmatrix}[4]{ \left( \begin{array}{cc}
 {\scriptstyle #1} & {\scriptstyle #2} \\ {\scriptstyle #3} &
 {\scriptstyle #4} \end{array} \right) }
\newcommand{\tmatrixb}[4]{ \left( \begin{array}{cc} #1 & #2 \\
 #3 & #4 \end{array} \right) }
\newcommand{\sqmatrix}[4]{\left[ \begin{array}{cc} #1 & #2 \\
 #3 & #4 \end{array} \right] }
\newcommand{\smsqmatrix}[4]{\mbox{\scriptsize $\left[ \begin{array}{cc}
 #1 & #2 \\ #3 & #4 \end{array} \right]$ \normalsize}}
\newcommand{\vct}[2]{ \left[ \begin{array}{c} #1 \\ #2 \end{array} \right] }

\newcommand{\smvct}[2]{\mbox{\footnotesize $\left[ \begin{array}{c} #1 \\
  #2 \end{array} \right]$ \normalsize} }

\newcommand{\smrow}[2]{\mbox{\footnotesize $\left[ \begin{array}{cc} #1 &
  #2 \end{array} \right]$ \normalsize} }

\newcommand{\rowvct}[2]{\left[ \begin{array}{cc} #1 &
  #2 \end{array} \right] }

%\newtheorem{theorem}{Theorem}
%\newtheorem{lemma}[theorem]{Lemma}
%\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{fact}{Fact}
\newtheorem{assumption}{Assumption}
\newtheorem{claim}{Claim}
%\newtheorem{definition}{Definition}
%\newtheorem{remark}{Remark}

% \newenvironment{proof}{ \begin{list}{\bf Proof:}{\setlength{\leftmargin}{0.5\leftmargin} \setlength{\labelwidth}{0.1in} }
% \item \slshape }{\hfill \rule{3mm}{3mm} \end{list}
% \vspace*{1ex}}

